Evaluation of a Bundling Technique for Parallel Coordinates

We describe a technique for bundled curve representations in parallel-coordinates plots and present a controlled user study evaluating their effectiveness. Replacing the traditional C^0 polygonal lines by C^1 continuous piecewise Bezier curves makes it easier to visually trace data points through each coordinate axis. The resulting Bezier curves can then be bundled to visualize data with given cluster structures. Curve bundles are efficient to compute, provide visual separation between data clusters, reduce visual clutter, and present a clearer overview of the dataset. A controlled user study with 14 participants confirmed the effectiveness of curve bundling for parallel-coordinates visualization: 1) compared to polygonal lines, it is equally capable of revealing correlations between neighboring data attributes; 2) its geometric cues can be effective in displaying cluster information. For some datasets curve bundling allows the color perceptual channel to be applied to other data attributes, while for complex cluster patterns, bundling and color can represent clustering far more clearly than either alone.

==> future.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

Bundled curve parallel-coordinates plots are designed to alleviate some
longstanding limitations of traditional polyline plots and to geometrically
reveal cluster structures specified for the input data. Bundled curve plots are
constructed from piecewise cubic B{\'e}zier curves with control points
judiciously selected to ensure $C^1$ continuity; this can alleviate
the well-known cross-over problems for polyline plots without any additional
visual aid beyond curve geometry. Cluster structures in the data are emphasized
by curve bundling, pulling curves belonging to the same cluster toward their
cluster centroid. 
The greatest advantage of bundling is that a wide range
of views from abstract high-level to detailed low-level representations
are easily obtained by tuning the bundling strength.
The cluster centroids can further be uniformly distributed to
take advantage of the whole plot area and reduce line cluttering. For large
datasets, line density plots for each cluster can be employed to avoid the
potential over-plotting problem. As traditional parallel coordinates are a special
case of our technique, many established extensions and interaction techniques such as 
brushing-and-linking can be applied without further enhancements.

The user study conducted in this work supports the following conclusions:
Firstly, curve bundling is effective in
displaying clustering information purely based on geometry. 
As a consequence, the color
channel can be used for other attributes or, in the case of
complex cluster patterns, be used in concert with color.
%provides as
%effective an alternative for displaying clustering information as color.
%At the same time, 
Secondly, with a properly chosen bundling
strength, bundled curve plots retain the same strength as polyline
plots in revealing correlations between visualized variables.
Hence one of the core aspects of analysis using parallel coordinates
carries over using bundling.
%Both of
%these points are supported by results from our user study. 
%In addition,
%we do not need to combine colors with density plots to reveal inner
%structure of clusters, as done in previous work. Instead, adjusting
%bundling strength generates views of the datasets at different levels,
%providing a high-level overview or detailed structure of the
%clusters. 
%Of course, the visualization
%results with bundled curve plots can be
%enhanced with other known visualization schemes, such as filtering,
%brushing, or advanced color mapping.
%Julian: this has been said in the previous paragraph.

In future work, we plan to compare bundled curve plots to
polylines and other curve-based approaches, as well as other approaches
to visualizing cluster information. 
%\ednote{Does this still seem like a good idea?}
%Julian: I'd say yes.
The high effectiveness of curved plots
compared with polyline plots was not obvious. The results of our user study
might trigger further perceptual investigations of
variants of parallel-coordinates plots.  It could be the case that other
forms of parallel-coordinates plots might be even more effective than
bundled curves---not only for cluster visualization but other
applications.

Qualitative improvements of this work are also possible. One problem
of interest is the automatic determination of the visualization parameters,
$\alpha$ and $\beta$, as well as the arrangement of cluster centroids,
guided by optimization criteria. For example, such criteria may
be related to a measure of line cluttering and curve smoothness. It is also
interesting to consider combining color mapping and curve density plots
selectively in order to further improve the high-level visualization of
clusters and low-level investigation of data items within each cluster.
%\ednote{What about interactive analysis?}
%\ednote{Deeper analysis of the geometry?}


==> related.tex <==
% !TEX root = infovis.tex
%-----------------------------------------------------------------

\section{Related Work}
\label{sec:related}

In parallel-coordinates visualization, points in $m$-dimensional space
are represented as lines crossing $m$ parallel axes in 2D, so there is
no inherent limit on dimensionality. The process of discovering
multivariate relations in a dataset is transformed to a 2D pattern
recognition problem. Parallel coordinates were introduced 
by Inselberg~\cite{Inselberg:1985:TPP,Inselberg:1990:PCT,Inselberg:2009:PC},
and extended by Wegman~\cite{Wegman:1990:HDA}.
%Recognizing the basic weakness of Cartesian plot as its inability to
%have more than three orthogonal coordinate axes, the
%parallel-coordinates idea is to give up orthogonality in favor of a
%system of parallel coordinate axes drawn in the two-dimensional plane
%so that there is no inherent limit on dimensionality. Each axis is
%subsequently labeled with a variable name and points on adjacent axes
%are connected with straight line segments to represent multidimensional
%data. The parallel-coordinates approach works well as a transform
%methodology for the unambiguous visualization of multivariate data and
%their relations.

Traditional parallel coordinates suffer from several problems,
especially for large datasets. One issue is the potentially heavy
over-plotting of lines, resulting in visual clutter. A proposed remedy
is to replace fully opaque, rasterized lines by a density
representation of the plotted
lines~\cite{Miller:1991:CLD,Wegman:1997:HDC}. This idea has been
adopted for frequency
plots~\cite{Rodrigues:2003:FPR}, gray-scale mappings in density
plots~\cite{Artero:2004:UCC}, and high-precision textures in
combination with transfer functions~\cite{Johansson:2005:RSC}.
For continuous data, line density can also be computed analytically using
an appropriate reconstruction kernel~\cite{Heinrich:2009:CPC}.

The cross-over problem for polylines arises when two or more lines share
common points on an axis. Several authors have solved this by using smooth
curves. Theisel~\cite{Theisel:2000:HOP} proposes a cubic B-splines model,
while Graham and Kennedy~\cite{Graham:2003:UCE} choose a quadratic or cubic
curve for a particular section depending on the shape formed by that section
and the two adjacent sections. Moustafa and Wegman~\cite{Moustafa:2006:MCD}
build smooth curves by replacing the piecewise linear interpolation of
polylines by interpolation via higher-order sinusoidal functions.
Holten~\cite{Holten:2010:ECIPDPV} adds a parameter to the spline-based
models~\cite{Graham:2003:UCE, Yuan:2009} to control the amount of smoothing.
All these techniques guarantee curve smoothness, alleviating the cross-over
problem by giving different trajectories to points that intersect at an
axis.  This allows the analyst to reliably connect the curves on either side
of the axis.


Visual clutter can also be reduced by preprocessing the data with a
clustering algorithm~\cite{Jain:1988:ACD}.
The clusters can then be displayed by extensions of
parallel coordinates~\cite{Fua:1999:HPC,Wegman:1997:HDC,Berthold:2003:TFS}.
Whereas early clustering work focused on reducing the amount of displayed data
by displaying only markers of entire clusters, recent work has instead focused
on displaying all the data and revealing details of the internal structure of
clusters. Johansson et al.~\cite{Johansson:2005:RSC} combine specific transfer
functions for density plots with feature animation, showing both an overview of
the data and the inner structure of its clusters. Novotny and
Hauser~\cite{Novotny:2006:OPF} extend such cluster-based parallel-coordinates
visualization to additionally display outliers and trends. 
Zhou~\cite{Zhou:2009:Splatting} detects clusters by splatting lines and applying a Gaussian
weight to proximate lines. 

Two recent publications~\cite{McDonnell:2008:IPC,Zhou:2008:VCP} enhance parallel-coordinates
plots following the same perceptual motivation of
geometric proximity as our method. Zhou et
al.~\cite{Zhou:2008:VCP} deform traditional polylines by applying attracting and repelling
forces. By construction, their method is based on proximity between the initial
polylines and, thus, achieves an implicit, yet fixed type of clustering. Their
method emphasizes the proximity of the polylines, rather
than showing externally provided clusters. Moreover, their
visual clustering is based on a piecewise model: the vicinity of polylines
between two neighboring data axes (or dimensions) of the
parallel-coordinates plot governs the visual clustering between those two data
dimensions; other pairs of neighboring data dimensions are clustered
independently. Therefore, high-dimensional data is not clustered on a
per-data-point level, but based on pairs of data dimensions. The
resulting visual clustering is thus sensitive to the order of data
dimensions in the parallel-coordinates plot.

Holten introduced edge bundling of tree layouts~\cite{Holten:2006:HEB}.
McDonnell and Mueller~\cite{McDonnell:2008:IPC} built on this idea, developing 
a geometric, spline-based approach to computing visual bundling that is similar to ours.
However, McDonnell and Mueller's technique has
a different objective: it targets illustrative parallel-coordinates
plots, using visual simplification and non-photorealistic rendering
techniques such as silhouette lines, halos, and shadows. Therefore, details of
the internal structure of data points within clusters are not a focus of
their research. Moreover, cluster membership information is still based on
color coding, whereas our approach provides a complementary,
geometry-based visualization of clusters.

Our method improves upon the
proximity-based parallel-coordinates techniques of McDonnell and
Mueller~\cite{McDonnell:2008:IPC} and Zhou et al.~\cite{Zhou:2008:VCP} in the
following ways. First, we make better use of the
available screen space by re-distributing visually clustered curves in a
uniform way. Therefore, there is much less overlap in the important parts of
the plots---in the regions between two data axes, where users identify
correlation of data points. In addition, overdraw and cluttering issues are
reduced by this redistribution. Second, we guarantee $C^1$
continuity of the curved lines across data axes, addressing the cross-over
problem.


%In 2005, Johansson \cite{Johansson:2005:RSC} proposed a new display
%technique by using high-precision structure texture for cluster
%visualization in PC. Except the high-level overview of the global
%structure of the whole dataset, using high-precision textures and
%different transfer functions could also reveal the inner structure
%of each cluster. With the similar objective, we address this problem
%using geometrical properties of B{\'e}zier curves. With the
%clustering information, by using a common or closed control points,
%B{\'e}izer curves will form curve bundles in PCs. The bundling
%technique is based on the principle of visually bundling curves
%belonging to the same cluster together analogous to the way
%electrical wires and network cables are merged into bundles along
%their joint paths and fanned our again at the end.

%The issue of visual clutter in large datasets can also be addressed by
%making use of interactive exploration. The interactive swapping of PC
%axes played an important role early on in order to explore the
%correlation between neighboring axes. Interaction can also be used to
%reduce the amount of displayed data by filtering or selection. For
%example, brushing-and-linking \cite{Becker:1987:BS}, known from scatter
%plots, is modified by Hauser et al.~\cite{Hauser:2002:ABE} to allow for
%angular brushing in parallel coordinates. Similarly, many of the
%aforementioned cluster-oriented visualization methods have relied on
%user input to highlight regions of the data representation.



%We share the basic motivation behind these techniques. However, our technique
%differs from previous work in its other goals and corresponding algorithmic
%realization: we target the visualization of large datasets, their associated
%cluster information, as well as the internal
%, both realized via the purely geometric approach of curve bundling.

%Curve bundles have been applied to visualization in a few previous papers.
%Balzer and Deussen~\cite{Balzer:2007:LDV} apply edge bundles to adjustable
%views of clustered graph layouts. Our bundling method is most related to the
%approach used for tree layouts of hierarchical data by
%Holten~\cite{Holten:2006:HEB}, where edge bundles of cubic B-splines are used
%to visualize adjacency relations in the hierarchies. We apply a similar method
%to the spatial layout in parallel coordinates.

%We might mention \cite{Bendix:2005:PSV}, maybe not.

There have been few previous papers providing user studies on parallel
coordinates.
%JH and those few papers are restricted to polyline plots. Li and Van
Jing~\cite{Jing:2007:JCFSPC} compares polyline parallel coordinates and scatterplots. 
Lanzenberger et al.~\cite{Lanzenberger:2005:EHS} investigate the
effectiveness of stardinates and parallel-coordinates plots applied to an
example data set with psychotherapeutic data. Henley et
al.~\cite{Henley:2007:VTGC} evaluate scatterplots and parallel coordinates for
the task of comparing genomic sequences. Ten Caat and
Roerdink~\cite{Caat:2007:TPC} study a tiled parallel-coordinates technique for
visualizing time-varying multichannel EEG data.  
Johansson et al.~\cite{Johansson:2008:PC} investigate the amount of noise that may be present
in parallel coordinates such that patterns can still be received.
Holten and van Wijk~\cite{Holten:2010:ECIPDPV} evaluate cluster identification performance for
curved and animated parallel coordinates, among others.
%JH Of these studies, only 
While Li and
van Wijk~\cite{Jing:2007:JCFSPC} examined the visualization of correlation for linear
parallel coordinates and Holten and van Wijk~\cite{Holten:2010:ECIPDPV} the visualization of clusters,
our user study %JH has a similar goal and uses a similar design.
aims at evaluating the impact of bundling and curves to the judgment of correlation and the
detection of clusters.

Finally, there seems to be no literature concerning the evaluation of bundling at all.





%-----------------------------------------------------------------

